CausalSpartanX: Causal Consistency and Non-Blocking Read-Only Transactions

Causal consistency is an intermediate consistency model that can be achieved together with high availability and performance requirements even in presence of network partitions. In the context of partitioned data stores, it has been shown that implicit dependency tracking using timestamps is more efficient than explicit dependency tracking. Existing time-based solutions depend on monotonic psychical clocks that are closely synchronized. These requirements make current protocols vulnerable to clock anomalies. In this paper, we propose a new time-based algorithm, CausalSpartanX, that instead of physical clocks, utilizes Hybrid Logical Clocks (HLCs). We show that using HLCs, without any overhead, we make the system robust on physical clock anomalies. This improvement is more significant in the context of query amplification, where a single query results in multiple GET/PUT operations. We also show that CausalSpartanX decreases the visibility latency for a given data item compared with existing time-based approaches. In turn, this reduces the completion time of collaborative applications where two clients accessing two different replicas edit same items of the data store. CausalSpartanX also provides causally consistent distributed read-only transactions. CausalSpartanX read-only transactions are non-blocking and require only one round of communication between the client and the servers. Also, the slowdowns of partitions that are unrelated to a transaction do not affect the performance of the transaction. Like previous protocols, CausalSpartanX assumes that a given client does not access more than one replica. We show that in presence of network partitions, this assumption (made in several other works) is essential if one were to provide causal consistency as well as immediate availability to local updates.

==> abstract.tex <==
\begin{abstract}
Causal consistency is an intermediate consistency model that can be achieved together with high availability and high-performance requirements even in presence of network partitions. In the context of partitioned data stores, it has been shown that implicit dependency tracking using clocks is more efficient than explicit dependency tracking by sending dependency check messages. Existing clock-based solutions depend on monotonic psychical clocks that are closely synchronized. These requirements make current protocols vulnerable to clock anomalies. 
%Existing work on causal consistency for replicated and partitioned data stores can be classified into those where partitions need to communicate with each other to check causal dependencies (e.g., COPS and Orbe), and those that rely on  synchronized clocks (e.g., GentleRain). The former suffer from high overhead resulted from high message complexity whereas the latter depend on clocks being monotonic and very closely synchronized. 
In this paper, we propose a new clock-based algorithm, \MYPROTOCOL, that instead of physical clocks, utilizes Hybrid Logical Clocks (HLCs).  We show that using HLCs, without any overhead, we make the system robust on physical clock anomalies. %When clocks are very tightly synchronized, the performance of \MYPROTOCOL is similar to that of GentleRain.} However, when clock skew is present, \MYPROTOCOL has substantially smaller latency of PUT operations. 
This improvement is more significant in the context of query amplification, where a single query results in multiple GET/PUT operations. 
%\MYPROTOCOL is unaffected by clock skew. By contrast, clock skew substantially affects the response time of GentleRain. 
%
We also show that \MYPROTOCOL decreases the visibility latency for a given data item comparing to existing clock-based approaches. In turn, this reduces the completion time of collaborative applications where two clients accessing two different replicas edit same items of the data store. {\color{blue} \MYPROTOCOL also provides causally consistent distributed read-only transactions. \MYPROTOCOL transactions need only one round of communication.} Like previous protocols, \MYPROTOCOL assumes that a given client does not access more than one replica. We show that in presence of network partitions, this assumption (made in several other works) is essential if one were to provide causal consistency as well as immediate availability to local updates.

\end{abstract}
\begin{IEEEkeywords}
Causal Consistency, Hybrid Logical Clocks, Distributed Data Stores, Key-value Stores, Geo-replication, Transactions
\end{IEEEkeywords} 




==> discussion_notused.tex <==
\section{Discussion: Why Hybrid Logical Clocks}
\label{sec:discussion}
The main property of logical clock proposed by Lamprot \cite{lamport} is that we can use logical clock to capture causality between events. Specifically, if event $e$ happens-before $f$ (see Definition \ref{def:happens}), then logical clock timestamp assigned to $e$ is smaller than logical clock timestamp assigned to $f$. Although logical clocks help us to capture causality between events, using them in the distributed data store system has some complications. First, as mentioned in \cite{gentleRain}, using logical clocks can cause clocks at different servers move at very different rates. Specifically, the logical clock of a server with higher event rate moves faster than the logical clock of a server with smaller event rate. When clocks of different servers moves at different speed, the visibility of update can be delayed arbitrary \cite{gentleRain}. Another problem of logical clocks is the timestamp assigned to version has not meaningful relation with a \textit{real clock}. Thus, if we use logical clocks for timestamping versions, we have no way to access a certain version of a key or snapshot of the system at the certain physical time. 

Physical clocks, on the other hand, do not have the above mentioned problem of logical locks. Specifically, they advance spontaneously. Thus, unlike logical clocks, even if no event occurs at a server, its clock advances by its own. Another advantage of physical clock is that if use them to timestamp versions, we can access the data of our system at a desired physical time. Although physical clocks have these benefits, they are not as efficient as logical clocks for capturing causal relation between events. In particular, if we timestamp events with physical clocks as soon as they occur, then it is not guaranteed that if event $e$ happens-before $f$ timestamp of $e$ is smaller than timestamp of $f$. To solve this problem, the approach of GentelRain is delaying write operations, but it can leads to increasing response time when clock synchronization is not good enough. Thus, it makes it sensitive on clock synchronization. 

Hybrid logical clocks combine the benefit of both logical clocks and physical clocks. Specifically, at one hand, just like physical clocks, it advances spontaneously, and it also is close to the real clock. On the other hand, without delaying event, it guarantees logical clock property that is if event $e$ happens-before $f$ timestamp of $e$ is smaller than timestamp of $f$. 

==> oldROTXRelated.tex <==
In \cite{snow}, Lu et. al. provided an interesting way to study read-only transactions based on four properties (called SNOW properties): 1) Strict serializability (S), 2) Non-blocking operations (N), 3) One response per read (O), and 4) coexistence with conflicting Write transactions (W). They have proved that it is impossible to have a read-only transaction that satisfies four of these requirements \cite{snow, newSnow}. Any algorithm that satisfies N + O is called \textit{latency-optimal} because it is as fast as possible. With this definition, CausalSpartanX is a latency-optimal causally consistent read-only transaction algorithm, because it is non-blocking and requires only one round of reading keys per transaction.  

Based on the tightness of the SNOW, any protocol that is not SNOW-optimal can be improved to become a SNOW-optimal algorithm. However, the strict serializability can not be achieved with availability in presence of network partitions. Specifically, the real-time requirement of strict serializability requires that if transaction $T1$ occurred after transaction $T2$ is done, then $T1$ must reflect the effect of transaction $T2$. Similar to the proof of CAP theorem \cite{cap}, it is straightforward to see it is impossible to guarantee this property if we want always-availability if $T1$ and $T2$ occurred in two different network partitions. 

Although snow-optimal protocol that includes strict serializability is not achievable with availability in presence of network partitions, we can achieve latency-optimality with availability even in presence of network partitions. Thus, any causally consistent distributed transaction algorithm that is not latency-optimal can become a latency-optimal algorithm. COPS-GT \cite{cops} is one example of such algorithm. COPS-GT \cite{cops} is a read-only transaction algorithm that only satisfies non-blocking property of SNOW properties. It may need a second round of reading key. Thus, it can be improved to become a latency-optimal protocol. Such improvement is provided in \cite{snow} called COPS-SNOW. Unlike COPS-GT, COPS-SNOW requires only one round making it a latency-optimal algorithm. COPS-SNOW achieves this by shifting complexity from read operations to write operations. 

Comparing to COPS-SNOW, CausalSpartanX has significantly smaller metadata. Specifically, in COPS-SNOW, for each version $X$, we need to store a list of all transactions that has read a version older than $X$. For each key, we also need to keep track of all transactions that has read the current version. Another problem of COPS-SNOW is doing explicit dependency check for every write operation. To do this explicit dependency check, nodes need to constantly communicate with each that increase the message complexity of the algorithm. CasualSpartanX does not have any these problem while providing the same latency-optimality of COPS-SNOW. 
%
%Our experimental results shows how CausalSpartanX performs better than COPS-SNOW considering the write-response time and throughput. 
%
%Similar to COPS-GT and COPS-SNOW, an improvement for Rococo \cite{rococo} called Rococo-SNOW is also provided in \cite{snow}. 

GentleRain \cite{gentleRain} read-only transaction algorithm is blocking \cite{gentleRain}. Also, it may need a second round of reading values. Thus, it does not satisfy any of SNOW properties. 
%
We saw that how using DSV in CausalSpartanX let us to make read-only transaction algorithm latency-optimal. 
Like GentleRain \cite{gentleRain}, Orbe \cite{orbe} and ChainReaction \cite{chainReaction} are both blocking algorithms that that need 2 or more round of reading key and they do not coexist with write transactions. Thus, they do not satisfy any of SNOW properties. 

Wren is a SNOW-optimal transactional causally consistent protocol. It is latency-optimal and also provides write transactions. It relies on client cash to provide a causally consistent snapshot. The significantly improves the throughput of transactions compared with non latency-optimal transactional systems such as Cure \cite{cure} that may need to block some write transactions. However, to achieve this, Wren increases the update visibility further up to 15\%. This increased latency can also occasionally becomes much higher in case of failures, that affects the tail latency \cite{book}.  
%
Regarding causal consistency, Wren keeps track of the dependencies of a version with two scalars; one for local updates and one for remote updates. This enable Wren to eliminate the GentleRain’s snapshot blocking. However, since all remote dependencies are tracked by a single scalar, like GentleRain, Wren still suffers from increased update visibility in cases of slow replicas (cf. Section \ref{sec:updatevis}).  Another issue with Wren is its requirement for the clients to cash the data that they have written in the system. It can be prohibitive for computationally-challenged clients such as mobile devices.



Occult \cite{occult} is another transactional causally consistent protocol. The main design goal of Occult is to decrease the update visibility. In fact, Occult pushes this direction to the end, and makes all the updates immediately visible for the clients. However, to achieve this, Occult scarifies the always-availability. Specifically, client may need to retries their read requests to get a causally consistent value of a key. This problem contradicts one of the most important features of the causal consistency that makes it favorable over stronger consistency models that is availability during network partitions. Another important problem of Occult is its single-leader replication policy. Specifically, all writes in the system must be done in a single replica. Occult uses this policy to manage its metadata overhead that is high in nature (i.e., in the order of the number of all partitions where clients can write) to avoid false positive causal consistency violation detection.
